Informable Multi-Objective and Multi-Directional RRT* System for Robot Path Planning

Multi-objective or multi-destination path planning is crucial for mobile robotics applications such as mobility as a service, robotics inspection, and electric vehicle charging for long trips. This work proposes an anytime iterative system to concurrently solve the multi-objective path planning problem and determine the visiting order of destinations. The system is comprised of an anytime informable multi-objective and multi-directional RRT* algorithm to form a simple connected graph, and a proposed solver that consists of an enhanced cheapest insertion algorithm and a genetic algorithm to solve the relaxed traveling salesman problem in polynomial time. Moreover, a list of waypoints is often provided for robotics inspection and vehicle routing so that the robot can preferentially visit certain equipment or areas of interest. We show that the proposed system can inherently incorporate such knowledge, and can navigate through challenging topology. The proposed anytime system is evaluated on large and complex graphs built for real-world driving applications. All implementations are coded in multi-threaded C++ and are available at: https://github.com/UMich-BipedLab/IMOMD-RRTStar.

==> IMOMTvsTSPvsCarPooling.tex <==
% \section{Car-Pooling/Ride-Sharing, Traveling Salesman Problem, and IMOMD-RRT\textsuperscript{*}}
% \label{sec:LiteratureComparison}
% This sections describes some essential difference among the three sets of problems. 
% 
% \textbf{1)} Problems such as car-pooling, ride-sharing, food delivery, or combining
% public transportation and car-pooling handle different types of constraints such as
% maximum seats, time window, battery cost, number of served requests along with
% multi-destinations\bh{cite}; and therefore are solved by Genetic Algorithms \bh{cite}
% or reinforcement learning \bh{cite}. In addition, they assume the graph/map with
% known distances between nodes is provided. 
% 
% 
% \textbf{2)} Traveling Salesman Problem (TSP), as mentioned in Sec.~\ref{sec:MO-TSP},
% is a NP-hard problem to find a shortest path that visits every node exactly once and
% return to the start node in a cyclic graph. However, 
% 
% 
% 
% 
% 
% \begin{figure}[t]%
%     \centering
%     \subfloat{%
%         \label{fig:Noncyclic}%
%         % l, b, r,t
%     \includegraphics[trim=0 0 0 0,clip,width=0.48\columnwidth]{placeholder.png}}~
%         \subfloat{%
%         \label{fig:BadHamiltonian}%
%         % l b r t
%     \includegraphics[trim=0 0 0 0,clip,width=0.48\columnwidth]{placeholder.png}}%
%     \caption[]{\bht{Hamiltonian path}
%     }%
% \label{fig:Hamiltonian}%
% \end{figure}
% 


==> Methods-pre.tex <==
\section{Multi-objecticves RRT$^\ast$}
\label{sec:Methods}
\bh{mention multi-directional RRT}

This section purposed an informable Multi-objective Multi-threading Rapidly-exploring Random Tree* as an efficient data structure and searching algorithm to quickly search on large-scale undirected weighted graph that meets the existence constraint (the solution path must passes by all the objectives at least once) and the order constraint (with fixed starting point and end point). The key idea is to first simplify the searching problem on the large-scale graph to the "one-stroke" problem base on small graph. 

\input{alg_morrt}

\subsection{Graph Simplifier}
This section provides some details of the implementation on how to simplify the path searching problem based on large graph to the path organizing problem based on the small graph using RRT* algorithm.


As shown in Algorithm \ref{alg:morrt}, from line 4 to line 12 is the graph simplifier part. The basic idea is that the algorithm put all the objectives, including the sources and target as the same into the goal set $\Gcal$. For each iteration [line 3 at Algorithm \ref{alg:morrt}], the MORRT will first sample a random node with higher sampling bias for the nodes from the goal set $\Gcal$ of the graph. 

\begin{remark} Sampling bias for MORRT algorithm is a bias in which that the nodes from the goal set $\Gcal$ of the graph has a higher probability to be selected as the random point. The purposed of this bias is to find a path between two different goals as soon as possible. 
\end{remark}

\input{alg_final_path}


After the random node $\nsub{rand}$ is selected, the MORRT would repeat RRT* for each objective $o_1$ in the goal set $\Gcal$: (1) [line 6] find the node $\nsub{parent\_candidate}$ in spanning tree of $o_1$ which has the minimum euclidean distance to random node $\nsub{rand}$. (2) [line 8-10] for all the neighbors of $\nsub{parent\_candidate}$ which has not been expanded by the spanning tree of $o_1$, find the $\nsub{child}$ which has minimum euclidean distance to the random node $\nsub{rand}$, thus insert and rewire. (3) [line 11-12] if the inserted node $\nsub{child}$ has already be expanded by other spanning tree of other objective $o_2$, then bond $o_1$ and $o_2$, meaning that a path from $o_1$ to $o_2$ is found. In some cases a path from $o_1$ to $o_2$ is found in the previous iteration, this step would update the path from  $o_1$ to $o_2$ to the shorter path.



\subsection{path organizer}
When the graph simplifier is run for multiple times, it is almost sure that path would be found between destinations. As the iteration number and the volume of spanning tree of each destination grows, it would be almost sure that a "union" among those destinations would be formed.


\begin{remark} Union is formed when all the destinations and the paths found by the graph simplifier forms a connected graph, meaning that starting from any objective, it is possible to reach any other destination with the given graph. 
\end{remark}

When the union is formed and under the assumption that there exists a path which starts at starting point $n_s$, ends at the terminating point $n_t$ and passes by all the rest of destinations, the path organizer would be able to determines the order of different destinations and find the best path within all the constraints. 


The basic idea is presented in Algorithm \ref{alg:final_path}: (1) [line 1-2] Use Breadth-First Search algorithm to first find a path $\Tcal$ from the starting point $n_s$ to the terminating point $n_t$, and put all the destinations on the path $\Tcal$ into a set $\Scal$. (2) [line 3-9] During each iteration, the path organizer would find the best destination to be inserted with minimum insertion distance and execute the corresponding insertion plan. The algorithm will keep running until all the destinations has been inserted to the path $\Tcal$.

\begin{remark} How to determine the insertion plan is shown in Algorithm \ref{alg:best_insert}. The input of the insertion planner is the current path $\Tcal$ and the potential node to be inserted $n_k$. First, we defined the notation $\| \cdot \|$ to be the travel distance between two destinations. Also, we have also defined two possible insertion methods: insertion in place (method 1) and insertion in sequence (method 2). The insertion in place (method 1) takes the node cursor $n_i$ on the path $\Tcal$ and the node to be inserted $n_k$ as input and calculated the additional travel cost to the inserted path $\Tcal$. In this case, the inserted path would insert the sequence $n_k,n_i$ right after the original $n_i$ in $\Tcal$, and the additional cost would be $2\|n_i-n_k\|$. The insertion in sequence (method 2) shared the input/output form with method 1. it differs with method 1 in that only $n_k$ will be inserted between $n_i$ and $n_{i+1}$ on the path, and the additional travel cost is calculated by  $ \| n_i- n_k\| + \| n_{i+1}- n_k\| - \| n_{i+1}- n_i\|$.
\end{remark}


After each iteration of the path organizer, one uncovered  destination will be added or inserted to the path $\Tcal$, by first find the insertion plan and additional travel distance (method 1 or method 2) for every uncovered destination with given path, then pick the insertion plan among all the uncovered destinations with minimum additional travel distance.


\input{alg_best_insert}

% \input{alg_rrt}
% \input{alg_choose_parent}
% \input{alg_rewire}


==> Methods.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% IMOMD RRT*
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Informable Multi-objecticve and Multi-directional RRT$^\ast$}
\label{sec:IMOMDRRT}
% \bh{mention multi-directional RRT, missing ChooseParent, ReWiring, CheckUnion,
% Neighbor seems wrong? Definition of Union?}
This section introduces an informable multi-objective and multi-directional
Rapidly-exploring Random Tree$^*$ (\imomdN) as an efficient data structure and
searching algorithm to quickly search on large-scale undirected weighted graph that
meets the existence constraint (the solution trajectory must passes by all the
objectives at least once), and the order constraint (with fixed starting point and
end point). In other words, the \imomd creates a union graph containing the
objectives, source, and target. Next, we proposed polynomial time solver to determine
the visiting order of nodes in the graph, see Sec.\ref{sec:WIBSFRTSP}.

% The key idea is to reduce the searching problem on the large-scale graph
% (the OSM) to the "one-stroke" problem base on small graph, which only consist of
% edges connecting objectives. 

\input{alg_morrt}


\subsection{Standard \rrt Algorithm}
The original \rrt\cite{RRTStar} is a sampling-base, incremental planner with
guaranteed asymptotic optimality in continuous configuration space. In general, \rrt
grows a tree where leaves are states connected by edges of linear path segments with
the minimal cost. Additionally, \rrt considers nearby nodes of a sample to choose the
best parent node and to rewire the graph if shorter path is possible to guarantee
asymptotic optimality.



\subsection{Multi-objective and Multi-directional \rrt on Graphs}
The proposed \imomd differs from the original \rrt in \add{five} aspects. First, the
sampling is performed by picking a random node in the graph. Second, \add{the
choose-parent step....} Third, \add{the rewiring step....}  Forth, in addition to
the source and the target node, each of the objectives grows its own tree; thus, it
leads to a family of trees. Lastly, if a node
belongs to more one tree, the trees will be merged, as shown in
Algorithm~\ref{alg:morrt}. 

\input{alg_rewire}

Our proposed graph-based \rrt modification is summarized below with notation that
generally follows Graph Theory~\cite{bondy1976graph}. A graph $\Gcal$ is an ordered
triple $(\Vcal(\Gcal), \Ecal(\Gcal), \Psi_\Gcal)$, where $\Vcal(\Gcal) = \{v=(x,y)~|~
x,y\in\reals\}$ is a nonempty set of nodes, $\Ecal(\Gcal)$ is a set of edges
(disjoint from $\Vcal(\Gcal)$), and an indication function $\Psi_\Gcal$ that
associates each edge of $\Gcal$ with an unordered pair (not necessarily distinct) of
nodes of $\Gcal$. 


Given a set of destinations $\Dcal = \{d_i|d_i\in\{v_s, v_t, \Ocal\}\}_{i =
1}^{M+2}$, where $v_s\in\Vcal(\Gcal)$ is the source node, $v_t\in\Vcal(\Gcal)$ is the
target node, and $\Ocal\subseteq\Vcal(\Gcal)$ is the set of objectives, the \imomd solves
the multi-objective planning problem by growing a tree $T(d_i) = (V, E)$, where
$V\subseteq\Vcal(\Gcal)$ is a vertex set of position connected by edges $E\subseteq\Ecal(\Gcal)$
at each of the destinations $d_i\in\Dcal$. Thus, it leads to a family of trees $\Tcal
= \{T(o_1), \cdots, T(o_M), T(v_s), T(v_t)\}$. 

\input{alg_update_union}


The proposed \rrt (Algorithm~\ref{alg:morrt}) explores the graph $\Gcal$ by random
sampling from vertices in $\Vcal(\Gcal)$ and extending nodes to grow each tree of
destinations. We explain a few important functions of \imomd below.

% \bh{How about ChooseParent and Rewire?}
% Considering nearby nodes of a sampled node to choose the best parent node and
% rewiring the graph guarantee asymptotic optimality
% (Algorithm~\bh{alg:rrtChooseParent} and \bh{alg:rrtRewire}), as with the classic
% algorithm. 


% \bh{This does not explain how to choose a parent but chose a parent candidate}
\bh{Check again}
\textit{1) Parent Choosing and Graph Rewiring:} Choosing the best parent node (line 9
in Algorithm \ref{alg:morrt}) and rewiring the graph (Algorithm \ref{alg:rewire})
guarantee asymptotic optimality, as with the classic algorithm. The parent candidate
$\vsub{parent\_candidate}$ is determined by finding a node in the spanning tree
$T(d_i)$ of the objective $d_i$ with the smallest euclidean distance to the random
node $\vsub{rand}$:

\begin{equation}
    \vsub{parent\_candidate} = \underset{v \in  T(d_i) }{\argmin}\| v - \vsub{rand}
    \|_2. 
\end{equation}
After a parent candidate is chosen, the nearby nodes are rewired if shorter paths are
found.

\input{algo_merge}


% \textit{2) Tree Merging:}\add{[Jenny: redundant paragraph (already covered by Union Checking (3))] } 


\textit{2) Union Checking:} The Disjoint-set data structure\bh{cite} is implemented
to examine the union of a graph. We summarize below for completeness, see \bh{cite}
for details.  The disjoint-set data structure supports three operations: (1) makes a
new vector $\Mcal$ containing all the destinations $d_i$, and initializes the
representative of each destination $d_i$ to be itself (line 3-5 in Algorithm
\ref{alg:morrt}); (2) finds the representative of the tree containing a given
element (Algorithm \ref{alg:update_union}); (3) merges the two trees (Algorithm
\ref{alg:merge}). To check whether a union is formed is equivalent to check whether
the representatives for all the trees are the same (Algorithm \ref{alg:union}).


Briefly speaking, if the inserted node $\nsub{child}$ has already
been expanded by other tree of objectives $T(d_{j})$, then $T(d_i)$ and $T(d_{j})$
are merged (i.e., a path from $d_i$ to $d_j$ is found). In some cases a path from
$d_i$ to $d_j$ is found in the previous iteration, this step would update the path
from  $d_i$ to $d_j$ to the shorter path.


\input{alg_union}

% \add{\href{https://www.semanticscholar.org/paper/An-improved-equivalence-algorithm-Galler-Fischer/3eed5bd2c67c8f8a44044f7defd7d245aa139647}{not sure..}}
% \add{copy from: \href{https://en.wikipedia.org/wiki/Disjoint-set_data_structure#cite_note-Galler1964-2}{Wikipedia}}





% Given a source node $v_s\in\Vcal(\Gcal)$ and a target node $v_t\in\Vcal(\Gcal$, and
% objectives ($\Ocal\in\Vcal(\Gcal$), the \imomd solves the multi-objective planning
% problem by growing a tree $T(d_i) = (V, E)$, where $V\in\Vcal(\Gcal)$ is a vertex set
% of position connected by edges $E\in\Ecal(\Gcal)$ at all destinations $\Dcal = \{v_s,
% v_t, \Ocal\}$. Briefly speaking, the proposed \rrt (Algorithm~\ref{alg:morrt})
% explores the graph $\Gcal$ by random sampling from
% vertices in $\Vcal$ and extending nodes to grow the trees.



% Considering nearby nodes of a sampled node to choose the best parent node and
% rewiring the graph guarantee asymptotic optimality
% (Algorithm~\bh{alg:rrtChooseParent} and \bh{alg:rrtRewire}), as with the classic
% algorithm. 

\begin{remark}
To facilitate faster convergence and to find better paths, we use sampling with a
goal bias, limited search space, and Gaussian sampling. For more details, see our
implementation on GitHub~\cite{githubFileIMOMD}.
\end{remark}


\subsection{Discussion of Informability}
\label{sec:Informable}
As mentioned in Sec.~\ref{sec:Intro}, robotics inspection considers prior knowledge of the inspection
trajectory, so that the robot can examine certain equipment or area of interests or avoid certain areas in a factory.
The prior knowledge can be naturally provided as a number of pseudo destinations in the \imomt to form a union graph, which is then
rewired by the \imomd to further shorten and improve the full trajectory of inspection. Note that in the process of rewiring, the pseudo destinations may be rewired so they no longer exists.

\begin{remark}
    One can decide if the order of the pseudo destinations should be fixed or even the pseudo destinations should be objectives (i.e., they will not be rewired in the rewiring process.).
\end{remark}



\input{alg_final_path}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% WI-BFS for R-TSP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Weighted Insertion BFS for Relaxed TSP}
\label{sec:WIBSFRTSP}
\bh{Check WI-BSF}
This section introduces a solver to solve the relaxed traveling salesman problem
(R-TSP) in polynomial time.


\subsection{Relaxed Traveling Salesman Problem}
\label{sec:RelaxedTSP}
The to-be-solved R-TSP differs from standard TSP\cite{applegate2011traveling, junger1995traveling,
punnen2007traveling} in two perspectives. First,
nodes are allowed to visit more than once, mentioned in Sec.~\ref{sec:MO-TSP}.
Second, we have a source node where we start and a target node where we end.
Therefore, the R-TSP can also be considered a relaxed Hamiltonian path
problem\cite{junger1995traveling, punnen2007traveling}.



\subsection{Weighted Insertion BFS}
\label{sec:WIBFS}
Under Definition~\ref{def:Union}, once all the destinations forms an union, there
exists a path that passes all destinations $\Dcal$ (i.e., a connected graph).
Therefore, it is indeed a relaxed R-TSP (see Sec.~\ref{sec:RelaxedTSP}), where we
have a source and target node as well as several objectives to be visited. We propose
a solver (Algorithm~\ref{alg:final_path}), called weighted insertion breadth-first
search (WI-BFS) with time complexity $O(N^3)$, to solve the R-TSP, where $N$ is the
cardinality of the destination set $\Dcal$. 

\begin{definition} 
    \label{def:Union}
    \bh{cite}The union of a graph is formed when all the destinations and the paths
    found by the \imomd forms a connected graph, which means starting from any
    objective, it is possible to reach any other destination. 
\end{definition}


We first leverage the BSF algorithm \bh{cite} to find a path $\Pcal$ from the source
$v_s$ to the target $v_t$. All the destinations $\Dcal$ on the path $\Pcal$ will be
put into a set $\Scal$. Next, during each iteration, an unexplored destination that
has the minimum distance, which is determined by Algorithm~\ref{alg:best_insert},
will be inserted to the path $\Pcal$. The algorithm runs until all the destinations
are inserted to the path (i.e., $|\Scal| = |\Dcal|$).



\begin{remark}
    $\Pcal$ is not a set because the elements inside are possibly duplicated. 
    Figure~\ref{fig:inplace} shows the duplicated case where $\Pcal = \{ d_s, \cdots,
    d_i, d_k, d_i, d_{i+1}, \cdots, d_t\}$, whereas fig.~\ref{fig:insequence}
    illustrates an unduplicated case where $\Pcal = \{ d_s, \cdots,
    d_i, d_k, d_{i+1}, \cdots, d_t\}$.
\end{remark}
% After every iteration of WI-BFS, one
% unexplored destination will be inserted to the path $\Pcal$. 


\begin{figure}[t]%
    \centering
    \subfloat{%
    \label{fig:inplace}%
    \includegraphics[trim=0 0 0 0,clip,width=0.48\columnwidth]{in_place.png}}~
    \subfloat{%
    \label{fig:insequence}%
    \includegraphics[trim=0 0 0 0,clip,width=0.48\columnwidth]{in_sequence.png}}%
    \caption[]{\bht{Insertion Plans}
    }%
    \label{fig:insertion}%
\end{figure}


Let the current sequence be $\Pcal_{\text{current}} = \{ d_{s},d_{1},
\cdots, d_{i},d_{i+1},\cdots, d_j, \cdots, d_{n}, d_{t}\}$ to indicate the visiting
order of destinations, where $d_{\{\cdot\}}\in\Dcal$. The travel cost $C(d_i,d_j)$ is
the sum of euclidean distance (provided by \imomdN) of the node sequence on the path
$\Pcal$: 
\begin{equation} 
    \label{def:distance} 
    \begin{aligned}
    C(d_i,d_j) = 
    &\sum_{m=1}^{k-1}\|n_m - n_{m+1}\|_2 +\|n_k - d_j\|_2 \\
    &+\|d_i - n_1\|_2.
    \end{aligned}
\end{equation}

Denote $\Kcal$ the set of destinations to be inserted. Let the to-be-inserted
destination be $d_k$ and its ancestor be $d_i$, where $d_k\in\Kcal$ and
$d_i\in\Pcal_\text{current}$. Where to insert $d_k$ and what the insertion distance
is on the current sequence $\Pcal_{\text{current}}$ is determined by
Algorithm~\ref{alg:best_insert} and is solved as follow: 
\begin{equation}
    F(\Pcal_\text{current}, d_k) =
    \underset{\underset{\underset{f\in{I_\text{in-place},I_\text{in-sequence}}}{d_i\in
    \Pcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k),
\end{equation}
where $I_\text{in-place}$ and $I_\text{in-sequence}$ are two insertion plans, and
are defined as

\textit{1) In-place Insertion:} This modifies the visiting sequence to 
$\Pcal_{\text{modified}} = \{ d_{s}, d_{1}, \cdots, d_{i}, d_{k}, d_{i}, d_{i+1},
\cdots, d_{n}, d_{t}\}$ by detouring from $d_{i}$ to $d_{k}$, as shown
in Fig.~\ref{fig:inplace}. Therefore, the insertion distance is 
\begin{equation}
    I_\text{in-place}(d_i,d_k)=2C(d_i,d_k).
\end{equation}

\textit{2) In-sequence Insertion:} 
    This modifies the visiting sequence to
    $\Pcal_{\text{modified}} = \{ d_{s}, d_{1}, \cdots, d_{i}, d_{k}, d_{i+1},
    \cdots, d_{n}, d_{t}\}$ by inserting $d_{k}$ between $d_{i}$ and $d_{i+1}$, as
    shown in Fig.~\ref{fig:insequence}. Therefore, the insertion distance is
\begin{equation}
    \begin{aligned}
        I_\text{in-sequence}(d_i,d_k)&=C(d_i,d_k)+C(d_{i+1},d_k) \\ 
                                     &- C(d_{i+1},d_i).
    \end{aligned}
\end{equation}

% \begin{equation}
%     \underset{d_i\in\Pcal_\text{current}}{\min} \{I_{\text{in-place}}(d_i,d_k), I_{\text{in-sequence}}(d_i,d_k)\}
% \end{equation}






% Let \bh{the specified insertion node in the current visiting sequence} and the
% to-be-inserted destination be $d_i$ and $d_k$, respectively, where $d_i\in
% \Pcal_{\text{current}}$ and $d_k\in\Ocal/\Scal$. We define two insertion methods to
% compute the insertion cost. 
% 
% \bh{Do we use $I$ before?}
% 
% 
% 
% Where in the sequence $Pcal$ and how to insert (in-place or in-sequence) the
% to-be-inserted node $d_k$ is determined by Algorithm~\ref{alg:best_insert}: 
% \begin{equation}
%     \underset{\underset{\underset{f\in{I_\text{in-place},I_\text{in-sequence}}}{d_i\in
%     \Pcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k),
% \end{equation}


% (insertion position, insertion method) pair for the given destination to be inserted
% $d_k$ with minimum insertion cost. The
% insertion planning solves the problem with the following generic formulation:
% \begin{equation}
%     \underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in
%     \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)
% \end{equation}

Finally, the WI-BFS algorithm solves the R-TSP problem by the following
\begin{equation}
    \underset{\underset{d_k\in\Kcal}{d_k,f}}{\min} \left[F(\Pcal_\text{current},
        d_k)\right] =
        \underset{\underset{d_k\in\Kcal}{d_k,f}}{\min}\left[\underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in
    \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)\right].
\end{equation}


% The SolveRTSP algorithm runs
% the inserting planning for every potential destination $d_k\in\Kcal$ and greedly
% finds out the (potential destination, insertion method) with the minimum insertion
% cost. The problem solved by SolveRTSP has larger scope than the insertion planning:
% \begin{equation}
%     \underset{\underset{d_k\in\Kcal}{d_k,f}}{\min}\left[\underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in
%     \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)\right]
% \end{equation}


% \begin{remark} 
%     How to determine the insertion plan is shown in Algorithm \ref{alg:best_insert}.
% The input of the insertion planner is the current path $\Tcal$ and the potential node
% to be inserted $n_k$. First, we defined the notation $\| \cdot \|$ to be the travel
% distance between two destinations. Also, we have also defined two possible insertion
% methods: insertion in place (method 1) and insertion in sequence (method 2). The
% insertion in place (method 1) takes the node cursor $n_i$ on the path $\Tcal$ and the
% node to be inserted $n_k$ as input and calculated the additional travel cost to the
% inserted path $\Tcal$. In this case, the inserted path would insert the sequence
% $n_k,n_i$ right after the original $n_i$ in $\Tcal$, and the additional cost would be
% $2\|n_i-n_k\|$. The insertion in sequence (method 2) shared the input/output form
% with method 1. it differs with method 1 in that only $n_k$ will be inserted between
% $n_i$ and $n_{i+1}$ on the path, and the additional travel cost is calculated by  $
% \| n_i- n_k\| + \| n_{i+1}- n_k\| - \| n_{i+1}- n_i\|$. 
% \end{remark}



% After each iteration of SolveRTSP, one uncovered destination will be added or
% inserted to the path $\Tcal$, by first find the insertion plan and additional travel
% distance (in-place or in-sequence insertion) for every uncovered destination with
% given path, then pick the insertion plan among all the uncovered destinations with
% minimum additional travel distance.


\input{alg_best_insert}

% \input{alg_rrt}
% \input{alg_choose_parent}
% \input{alg_rewire}






% Let the current visiting sequence be $\Pcal_{\text{current}} = \{ d_{s},d_{1},
% \cdots, d_{i},d_{i+1},\cdots, d_j, \cdots, d_{n}, d_{t}\}$ to indicate the order of
% destinations, where $d_{\{\cdot\}}\in\Dcal$. The travel cost $C(d_i,d_j)$ is the sum
% of euclidean distance (provided by \imomdN) of the node sequence on the path $\Pcal$:
% \begin{equation} 
%     \label{def:distance} 
%     C(d_i,d_j) = \|d_i - n_1\|_2  +
%     \sum_{m=1}^{k-1}\|n_m - n_{m+1}\|_2 +\|n_k - d_j\|_2. 
% \end{equation}
% 
% Let \bh{the specified insertion node in the current visiting sequence} and the
% destination to be inserted be $d_i$ and $d_k$, respectively, where $d_i\in \Pcal_{\text{current}}$ and $d_k\in\Ocal/\Scal$
% , and the destination to be inserted $d_k$. 
% 
% We define two insertion methods to compute the insertion cost with the specified
% insertion node in the current visiting sequence $d_i \in \Pcal_{\text{current}}$ 
% , and the destination to be inserted $d_k$. 
% 
% 
% \begin{enumerate}
%     \item{$f_1:$} The in-place insertion would modified the visiting sequence to be $\Pcal_{\text{modified}} = \{ d_{s},d_{1}...d_{i},d_{k},d_{i},d_{i+1}...d_{n}, d_{t}\}$ by detouring from $d_{i}$ to $d_{k}$.
%     $$f_1(d_i,d_k)=2\times C(d_i,d_k)$$
%     \item{$f_2:$} The in-sequence insertion would modified the visiting sequence to be $\Pcal_{\text{modified}} = \{ d_{s},d_{1}...d_{i},d_{k},d_{i+1}...d_{n}, d_{t}\}$ by inserting $d_{k}$ between $d_{i}$ and $d_{i+1}$.
%     $$f_2(d_i,d_k)=C(d_i,d_k)+C(d_{i+1},d_k) - C(d_{i+1},d_i)$$
% 
% \end{enumerate}
% 
% \textit{2) Insertion Planning: } The insertion planning is shown in Algorithm~\ref{alg:best_insert} by finding the (insertion position, insertion method) pair for the given destination to be inserted $d_k$ with minimum insertion cost. The insertion planning solves the problem with the following generic formulation:
% $$\underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)$$
% 
% Let $\Kcal$ be the set of destinations to be inserted. The SolveRTSP algorithm runs the inserting planning for every potential destination $d_k\in\Kcal$ and greedly finds out the (potential destination, insertion method) with the minimum insertion cost. The problem solved by SolveRTSP has larger scope than the insertion planning:
% $$\underset{\underset{d_k\in\Kcal}{d_k,f}}{\min}\left[\underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)\right]$$
















% The relaxed traveling salesman problem (R-TSP) differs from standard TSP\bh{cite} in
% two perspectives. First, a node is allowed to visit more than once, mentioned in
% Sec.~\ref{sec:MO-TSP}. Second, we have a source node where we start and
% a target node where we end. It can also be considered a relaxed Hamiltonian path
% problem\bh{cite}.
% 
% 
% 
% Under Definition~\ref{def:Union}, once all the destinations forms an union, there
% exists a path that pass all destinations $\Dcal$. Therefore, it is a relaxed
% traveling salesman problem (R-TSP) where we have a source and target node as well as
% several objectives to be visited. This section introduces an algorithm
% (Algorithm~\ref{alg:final_path}) based on Breadth-First Search (BFS)\bh{cite} with
% time complexity $O(N^3)$ to solve the R-TSP, where $N$ is the cardinality of the
% destination set $\Dcal$.
% 
% 
% \begin{definition}
%     \label{def:Union}
%     \bh{cite}A union is formed when all the destinations and the paths found by the
%     \imomd forms a connected graph, which means starting from any objective, it is
%     possible to reach any other destination with the given graph.
% \end{definition}
% 
% 
% We first leverage the BSF algorithm to find a path $\Pcal$ from the source $v_s$ to
% the target $v_t$, and put all the destinations $\Ocal$ on the path $\Pcal$ into a set
% $\Scal$. Next, during each iteration, the proposed algorithm  finds the best
% destination to be inserted with minimum insertion distance provided by \imomd (line
% 3-10, Algorithm~\ref{alg:final_path}), and executes the corresponding insertion plan.
% The algorithm runs until all the destinations are inserted to the path $\Pcal$.
% 
% 
% Let the path connecting $d_i$ and $d_j$ to be $\Pcal = \{d_i, n_1, n_2,...,n_k,d_j
% \}$, then the travel cost $L(d_i,d_j)$ is defined to be the sum of euclidean distance
% of the node sequence on the path $\Pcal$:
% \begin{Equation}
%     \label{def:distance}
%     L(d_i,d_j) = \|d_i - n_1\|_2  + \sum_{m=1}^{k-1}\|n_m - n_{m+1}\|_2 +\|n_k - d_j\|_2
% \end{Equation}
% 
% \textit{1) In-place Inserting and In-sequence Inserting: }Given the current visiting sequence $\Tcal_{\text{current}} = \{ d_{s},d_{1}...d_{i},d_{i+1}...d_{z}, d_{n}\}$ indicating the order of destinations, where $d\in\Dcal$ is the destination. The algorithm proposed two insertion methods to calculate insertion cost with specified insertion position $d_i \in \Tcal_{\text{current}}$ in the current visiting sequence and the destination to be inserted $d_k$:
% \begin{enumerate}
%     \item{$f_1:$} The in-place insertion would modified the visiting sequence to be $\Tcal_{\text{modified}} = \{ d_{s},d_{1}...d_{i},d_{k},d_{i},d_{i+1}...d_{n}, d_{t}\}$ by detouring from $d_{i}$ to $d_{k}$.
%     $$f_1(d_i,d_k)=2\times L(d_i,d_k)$$
%     \item{$f_2:$} The in-sequence insertion would modified the visiting sequence to be $\Tcal_{\text{modified}} = \{ d_{s},d_{1}...d_{i},d_{k},d_{i+1}...d_{n}, d_{t}\}$ by inserting $d_{k}$ between $d_{i}$ and $d_{i+1}$.
%     $$f_2(d_i,d_k)=L(d_i,d_k)+L(d_{i+1},d_k) - L(d_{i+1},d_i)$$
% 
% \end{enumerate}
% 
% \textit{2) Insertion Planning: } The insertion planning is shown in Algorithm~\ref{alg:best_insert} by finding the (insertion position, insertion method) pair for the given destination to be inserted $d_k$ with minimum insertion cost. The insertion planning solves the problem with the following generic formulation:
% $$\underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)$$
% 
% Let $\Kcal$ be the set of destinations to be inserted. The SolveRTSP algorithm runs the inserting planning for every potential destination $d_k\in\Kcal$ and greedly finds out the (potential destination, insertion method) with the minimum insertion cost. The problem solved by SolveRTSP has larger scope than the insertion planning:
% $$\underset{\underset{d_k\in\Kcal}{d_k,f}}{\min}\left[\underset{\underset{\underset{f\in{f_1,f_2}}{d_i\in \Tcal_{\text{current}}}}{d_i,f}}{\min}f(d_i,d_k)\right]$$
% 
% After each iteration of SolveRTSP, one uncovered destination will be inserted to the path $\Pcal$ by brute force until all the destinations are covered.
% 
% % \begin{remark}
% %     How to determine the insertion plan is shown in Algorithm \ref{alg:best_insert}.
% % The input of the insertion planner is the current path $\Tcal$ and the potential node
% % to be inserted $n_k$. First, we defined the notation $\| \cdot \|$ to be the travel
% % distance between two destinations. Also, we have also defined two possible insertion
% % methods: insertion in place (method 1) and insertion in sequence (method 2). The
% % insertion in place (method 1) takes the node cursor $n_i$ on the path $\Tcal$ and the
% % node to be inserted $n_k$ as input and calculated the additional travel cost to the
% % inserted path $\Tcal$. In this case, the inserted path would insert the sequence
% % $n_k,n_i$ right after the original $n_i$ in $\Tcal$, and the additional cost would be
% % $2\|n_i-n_k\|$. The insertion in sequence (method 2) shared the input/output form
% % with method 1. it differs with method 1 in that only $n_k$ will be inserted between
% % $n_i$ and $n_{i+1}$ on the path, and the additional travel cost is calculated by  $
% % \| n_i- n_k\| + \| n_{i+1}- n_k\| - \| n_{i+1}- n_i\|$.
% % \end{remark}
% 
% 
% 
% % After each iteration of SolveRTSP, one uncovered destination will be added or
% % inserted to the path $\Tcal$, by first find the insertion plan and additional travel
% % distance (in-place or in-sequence insertion) for every uncovered destination with
% % given path, then pick the insertion plan among all the uncovered destinations with
% % minimum additional travel distance.
% 
% 
% \input{alg_best_insert}
% 
% % \input{alg_rrt}
% % \input{alg_choose_parent}
% % \input{alg_rewire}
% 


==> Related-Work-pre.tex <==
\section{Related Work}
\label{sec:RelatedWork}
Multi-goal path planning in a given graph requires constructing a feasible path and determining the sequence of intermediate destinations to visit. In this section, we review the variants of path planning algorithms and several types of multi-goal path planning problems and finally summarize our main contributions.

\subsection{Sampling-Based Planning in Discrete Space}
Discrete motion planning is an algorithm to solve the classical problem that finding the shortest path from a starting point to a destination in discrete configuration space. There are traditional Dijkstra, A* algorithms 

There are many variants of A* to improve the speed up the computing time.
Inflating the heuristic value makes the A* algorithm likely to expand the nodes that close to the goal. It trade-off between computing time and the quality of solution, but the solution bounds on sub-optimality.
Anytime Repairing A* (ARA*) algorithm implemented weighted A* and keep decrease the weight parameter every iteration.
As it decrease the weight parameter every iteration, ANA* keep find the better solition as we compute longer.
Anytime Non-parametric A* (ANA*) works similar to ARA*, 

R*

Jumping Point Search (JPS) algorithm

Bidirectional A*
\bh{cite}
In high-dimensional spaces, discrete planning has difficulties for run-time and memory because of the increment of successors. The sampling-based planning algorithms, mostly well-known Rapidly-exploring Random Tree(RRT)\cite{VanillaRRT}, have been stands out for its low complexity and high efficiency in exploring high-dimensional and continuous configurations spaces.

Recently, the sampling-based planning algorithm have begun to be implemented to discrete space.
RRLT dRRT*

As a large branching factors in discrete  , discrete search method become sampling-based discrete planner

\subsection{Multi-goal path planning}
The multi-goal path planning is a task to find a feasible path connecting several destinations. Multi-goal path planning can be decoupled into two tasks: one is to find the sequence of destinations to be visited that minimize the travel cost, and the other task is to find feasible paths that connect the destinations in the determined order.

To solve the TSP, paths between all pairs of target need to be computed to identify the distance matrix for TSP. It takes $ \frac{(n+2)(n+1)}{2} $ times of path planning algorithm, which is time-consuming. 

Expanding multiple trees using RRT for multi destinations problem was introduced in \cite{devaurs2014multi}. The RRT trees are rooted at starting point, terminating point, and every intermediate destinations. 
The only one tree is selected in every iterations, and it expands to the random sample based on the RRT algorithms.
When any two trees are approach each other close enough, we could merge the two trees into one \cite{devaurs2014multi} or generating a 'virtual' connection keeping two trees separately \cite{janovs2021multi, vonasek2019space}
The last method increase the opportunity to find a more optimal path between the two trees.

The combinatorial problem determining the order of multiple targets is usually considered as an Traveling Salesman Problem (TSP). The TSP is a classic NP-hard problem about finding a shortest possible cycle that visits every goals exactly once and return to the starting point. The objective of this paper is to find the shortest path that visits multiple intermediate destinations with a given start-point and end-point. In a graph $ G = (V, E) $ with fixed starting point $v_s$ and terminating point $v_t$, the shortest path from $v_s$ to $v_t$ visiting each node of V exactly once is called the shortest Hamiltonian path. The shortest Hamiltonian path can be solved as a standard TSP problem by changing the cost $ C(v_s, v_t) $ into $ -M $ \cite{junger1995traveling, punnen2007traveling}

In real-world such as route planning for car, however, there is no reason to have a constraint that each node have to be visited exactly once. As shown in Fig. , if nodes were allowed to visited more than once, it is possible to find a feasible path in the graph which doesn't have the Hamiltonian path. Moreover, without the constraints in the graph, the shortest Hamiltonian path cannot guarantee the shortest path from $v_s$ to $v_t$ visiting every intermediate node as shown in fig.

\subsection{Contributions}


==> SFNY.tex <==
\begin{table}[!t]
\caption{}
\label{tab:SFNY}
\begin{tabular}{|c|c|c|c|}
\hline
            & San Francisco & New York & Chicago \\ \hline
\# of Nodes &               &          &         \\ \hline
\# of Edges &               &          &         \\ \hline
\end{tabular}
\end{table}


==> alg_best_insert.tex <==
\begin{algorithm}[!tbp]
    \caption{BestInsertionPlan($\Scal, d_k$)}
\label{alg:best_insert}

    \For {$s_i \in \Scal$}
        {
        $\ell_1  \leftarrow \lambda_\text{in-place}(p_i, d_k)$;

        \If{$s_i = \Scal_\text{last\_node}$ }
            {
            % distance\textsubscript{2} $\leftarrow $ distance\textsubscript{1};
            $\ell_\text{local\_min} \leftarrow  \ell_1$;

            $\text{plan}_\text{local\_min} \leftarrow \text{in-place insertion}$
            }
        \Else
            {
            $\ell_2 \leftarrow I_\text{in-sequence} (p_i, d_k)$;
            
            \dl{add}
            
            $\ell_3 \leftarrow I_\text{swapping-left} (p_i, d_k)$;
            
            $\ell_4 \leftarrow I_\text{swapping-right} (p_i, d_k)$;
            
            $\ell_5 \leftarrow I_\text{swapping-both} (p_i, d_k)$;
            
            \dl{modify}
            
            $\ell_\text{local\_min} \leftarrow  \min({\ell_1, \ell_2, \ell_3, \ell_4, \ell_5})$;
            
            $\text{plan}_\text{local\_min} \leftarrow \underset{\text{plan[j]} \in  \{1,2,3,4,5\} }{\argmin} \ell\textsubscript{$j$};$

            \If{$\ell_1 < \ell_2$}{
                $\ell_\text{local\_min} \leftarrow  \ell_1$;

                $\text{plan}_\text{local\_min} \leftarrow \text{in-place insertion}$
            }
            \Else{
                $\ell_\text{local\_min} \leftarrow  \ell_2$;

                $\text{plan}_\text{local\_min} \leftarrow \text{in-sequence insertion}$
            }

            }%else
        \dl{modify $\ell_\text{local\_min} < \ell_\text{global\_min}$}
        
        % \If{$\ell_\text{global\_min} < \ell_\text{local\_min}$}{
        % $\ell_\text{global\_min} \leftarrow \ell_\text{local\_min}$;
        % $\text{plan}_\text{global\_min} \leftarrow \text{plan}_\text{local\_min}$;
        % }

}
        % \If{distance\textsubscript{global_minimum}}{}
        % \Else{}
        % Opt\textsubscript{plan}$[i] \leftarrow \underset{j \in  \{ 1,2\} }{\argmin}$ distance\textsubscript{$j$};

        % Opt\textsubscript{dis}$[i] \leftarrow$ distance\textsubscript{Opt\textsubscript{plan}$[i]$};
        % }
        % dis $\leftarrow \min$  Opt\textsubscript{dis};


    return $\ell_\text{global\_min},\text{plan}_\text{global\_min}$;
\end{algorithm}



==> alg_choose_parent.tex <==
\begin{algorithm}[!htbp]
    \caption{\scalebox{0.95}{$\nsub{parent}\leftarrow$ ChooseParent($\Ncal_T, \nsub{nearest}, \nsub{new}$)}}
\label{alg:rrtParent}
    $\nsub{parent}\leftarrow\nsub{nearest}$

    $\csub{parent}\leftarrow$ Cost($\nsub{nearest}$)  $+$ c$(\nsub{nearest}, \nsub{new})$


\For{$n_{\text{near}} \in \Ncal_T$}
{
        $\traj^\prime\leftarrow$Steer$(\nsub{near}, \nsub{new})$

        \If{ObstacleFree($\traj^\prime$)}
        {
            $c^\prime = \text{Cost}(\nsub{near}) + c(\nsub{near}, \nsub{new})$

            \If{$c^\prime < \text{Cost}(\nsub{new})$ and $c^\prime < \csub{parent}$}
            {
                $\nsub{parent} \leftarrow \nsub{near}$

                $\csub{parent} \leftarrow c^\prime$
            }
        }
}
\Return $\nsub{parent}$
\end{algorithm}



==> alg_final_path.tex <==
\begin{algorithm}[!tbp]
    \caption{$\Pcal = (V,E) \leftarrow$ WI-BSF($\vsub{s}, \vsub{t}, \Ocal$)}
\label{alg:final_path}
    $\Pcal \leftarrow $ BFS($\vsub{s}$, $\vsub{t}$);
    
    $\Scal \leftarrow \{ \Pcal \}$;
    
    \While{$|\Scal| \neq |\Ocal|$}
    {
    
        $\Kcal \leftarrow \Ocal /\Scal$;
        
        % $\Ical \leftarrow $ [($\Pcal,j$) for $j \in \Kcal$];
        
        % $Dis,Plan \leftarrow $ Map($\mathtt{BestInsertPlan}, \Ical$);
        
        $\text{Dis}, \text{Plan} \leftarrow \mathtt{Vector}(),\mathtt{Vector}()$;
        
        \For{$d_k\in \Kcal$}
        {
            $\text{Dis}[d_k], \text{Plan}[d_k] \leftarrow \mathtt{BestInsertionPlan}(\Pcal, 
            d_k)$
        }
        
        $d_o \leftarrow \underset{d_j \in \Kcal}{\argmin}~\text{Dis}[d_j]$;
        
        $\Tcal \leftarrow $Execute($\Tcal,\text{Plan}[d_o]$);
        
        $\Scal \leftarrow $Insert($\Scal,d_o$);
        
    }
    
    \dl{It should return $\Scal$}
    return $\Pcal$;
\end{algorithm}


==> alg_morrt.tex <==
\begin{algorithm}[!tb]
    \caption{\\$\Tcal = (V,E) \leftarrow$ \imomd $(\vsub{s}, \vsub{t}, \Ocal, \Gcal)$}
    \label{alg:morrt}
    $\Tcal \leftarrow \mathtt{Initialize()}$;
    
    $ \Dcal \leftarrow$ $\{\vsub{s}, \vsub{t}\} \cup \{\Ocal\}$;
    
    $ \Mcal \leftarrow \mathtt{Vector}()$;
    
\For{$d_i$ $\in$ $\Dcal$}
{
    $ \Mcal[ d_i ] \leftarrow d_i$;
}
    
\While{True}
{
    $\vsub{rand}\leftarrow \mathtt{BiasedSampling}(\Gcal)$;
    
    \For{$d_i$ $\in$ $\Dcal$}
    {
        $\vsub{parent\_candidate}\leftarrow \mathtt{NearestLeaf}(T(d_i)$);
        
        $\Ncal \leftarrow \mathtt{Neighbor}(\vsub{parent\_candidate}) \cap~T(d_i)^\complement$;
        
        $\nsub{child}\leftarrow \underset{n \in  \Ncal }{\argmin} \| n-\vsub{rand} \|_2$ ;
        
        $T(d_i)\leftarrow \mathtt{Insert}(\nsub{child})$;

        $T(d_i)\leftarrow \mathtt{Rewire}(\nsub{child})$;
        
        \If{$\nsub{child} \in  T(d_j), d_j \in \Dcal/\{d_i \}$ } 
        {
            $\Mcal \leftarrow \mathtt{Merge}(\Mcal,T(d_i), T(d_j))$;
        }
        
    }%end for
    
    \If{$\mathtt{CheckUnion()}$}
    {
        
            $\Tcal \leftarrow \mathtt{SolveRTSP}(v_s,v_t,\Ocal)$;

    }
}%end while
\end{algorithm}

==> alg_rewire.tex <==
\begin{algorithm}[b]
    \caption{$\Tcal(d_{j}) \leftarrow$ 
             ReWire$(\Tcal(d_{j}), \nsub{child})$}
\label{alg:rewire}

$\Qcal \leftarrow \mathtt{Neighbor}(\nsub{child}) \cap \Tcal$;


$\nsub{parent} = \underset{n \in  \Pcal }{\argmin} \{\|d_j - n \| + \| n-\nsub{child}\|_2\}$; \bh{Per Dongmyeong: Cost(n) + $\norm{n - n_{child}}$}

$\Tcal \leftarrow \mathtt{Connect}(\Tcal,\nsub{parent}, \nsub{child})$


\For{$v \in \Qcal$}
{
    \If{$\|d_j - \nsub{child} \| + \|\nsub{child} - v \|_2 < \|d_j - v \|$} 
    {
        $\Tcal \leftarrow \mathtt{ReConnect}(\Tcal, \nsub{child}, v)$;
    }
}
    \Return $\Tcal$
\end{algorithm}


==> alg_rrt.tex <==
\begin{algorithm}[t]
    \caption{$\Tcal = (V,E) \leftarrow$ Omnidirectional CLF \rrt}
\label{alg:rrt}
    $\Tcal \leftarrow$ InitializeTree();

    $\Tcal \leftarrow$ InsertNode($\emptyset, \nsub{init}, \Tcal$);

\For{i=1 \KwTo $N$}
{
    $\nsub{rand}\leftarrow$ Sample($i$)

    $\nsub{nearest}\leftarrow$ Nearest($\Tcal, \nsub{rand}$)

    $(\nsub{new}, \traj^\prime) \leftarrow$ Extend($\nsub{nearest}, \nsub{rand},
    \kappa$)

    \If{ObstacleFree($\traj^\prime$)}
        {
            $\Ncal_T \leftarrow$ NearTo($\Tcal, \nsub{new}, |V|$)

            $\nsub{min} \leftarrow$ ChooseParent($\Ncal_T, \nsub{nearest}, \nsub{new}$)

            $\Tcal \leftarrow$ InsertNode($\nsub{min}, \nsub{new}, \Tcal$)

            $\Ncal_F\leftarrow$ NearFrom($\Tcal, \nsub{new}, |V|$)
            
            $\Tcal\leftarrow$ ReWire($\Tcal, \Ncal_F, \nsub{min}, \nsub{new}$)

        }
}
\Return $\Tcal$
\end{algorithm}



==> alg_union.tex <==
\begin{algorithm}[b]
    \caption{$\text{isConnected} \leftarrow$ 
             CheckConnectivity$(\Mcal,\Dcal)$}
\label{alg:union}

$\Lcal \leftarrow \mathtt{Set}()$;

\For{$d_i \in \Dcal$}
{
    $\Lcal\leftarrow\Lcal\cup\Mcal[d_i]$;
}

\If{$|\Lcal|=1$}
{
    $\text{isConnected} \leftarrow \text{True}$;
}
\Else{
    $\text{isConnected} \leftarrow \text{False}$;
}

    \Return $\text{isConnected}$
\end{algorithm}

==> alg_update_union.tex <==
\begin{algorithm}[b]
    \caption{$d_{parent} \leftarrow$ 
             UpdateConnectivity$(\Mcal , d)$}
\label{alg:update_union}

$d_{parent}\leftarrow d$;

\While{$\Mcal[d_{parent}] \neq d_{parent}$}
{
    $d_{parent}\leftarrow \Mcal[d_{parent}]$;
}

\While{$\Mcal[d] \neq d_{parent}$}
{
    $d_{iter} = \Mcal[d]$;
    
    $\Mcal[d] \leftarrow d$;
    
    $d \leftarrow d_{iter}$;

}

    \Return $d_{parent}$;
\end{algorithm}

==> algo_merge.tex <==
\begin{algorithm}[b]
    \caption{$\Mcal \leftarrow$ 
             Merge$(\Mcal,T(d_i), T(d_j))$}
\label{alg:merge}
    
$v_i \leftarrow \mathtt{UpdateConnctivity}(\Mcal,d_i)$;

$v_j \leftarrow \mathtt{UpdateConnctivity}(\Mcal,d_j)$;

\If{$v_i > v_j$}
{
    $\mathtt{swap}(v_i,v_j)$;
}

$\Mcal[v_j] \leftarrow v_i$;

% $\mathtt{UpdateConnctivity}(\Mcal,d_i)$;
$\mathtt{UpdateConnctivity}(\Mcal,d_j)$;

    \Return $\Mcal$
\end{algorithm}

==> tsp_complete_graph.tex <==
\begin{table}[]
\caption{Average Path Cost in Complete Graph}
\label{tab:Complete_avg_cost}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Order      & Insertion & Swap  & GA    & Swap+GA & BruteForce \\ \hline
5          & 1.005     & 1.000 & 1.000 & 1.000   & 1.000      \\ \hline
6          & 1.012     & 1.003 & 1.000 & 1.000   & 1.000      \\ \hline
7          & 1.020     & 1.008 & 1.000 & 1.000   & 1.000      \\ \hline
8          & 1.028     & 1.013 & 1.000 & 1.000   & 1.000      \\ \hline
9          & 1.038     & 1.018 & 1.000 & 1.000   & 1.000      \\ \hline
10         & 1.049     & 1.028 & 1.000 & 1.000   & 1.000      \\ \hline
11         & 1.055     & 1.033 & 1.000 & 1.000   & 1.000      \\ \hline
12         & 1.062     & 1.039 & 1.000 & 1.000   & 1.000      \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{Optimal Path ratio in Complete Graph}
\label{tab:Complete_optimal}
\begin{tabular}{|l|l|l|l|l|}
\hline
Order      & Insertion & Swap    & GA      & Swap+GA \\ \hline
5          & 89.867    & 100.000 & 100.000 & 100.000 \\ \hline
6          & 77.300    & 94.333  & 100.000 & 100.000 \\ \hline
7          & 64.433    & 84.167  & 100.000 & 100.000 \\ \hline
8          & 53.733    & 75.900  & 100.000 & 100.000 \\ \hline
9          & 41.800    & 66.300  & 100.000 & 100.000 \\ \hline
10         & 33.100    & 54.600  & 100.000 & 100.000 \\ \hline
11         & 26.071    & 48.233  & 99.958  & 99.958  \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{Standard Deviation of path cost ratio in Complete Graph}
\label{tab:Complete_std_diff}
\begin{tabular}{|l|l|l|l|l|}
\hline
Order      & Insertion & Swap  & GA    & Swap+GA \\ \hline
5          & 0.018     & 0.000 & 0.000 & 0.000   \\ \hline
6          & 0.030     & 0.013 & 0.000 & 0.000   \\ \hline
7          & 0.038     & 0.023 & 0.000 & 0.000   \\ \hline
8          & 0.046     & 0.032 & 0.000 & 0.000   \\ \hline
9          & 0.053     & 0.037 & 0.000 & 0.000   \\ \hline
10         & 0.060     & 0.047 & 0.000 & 0.000   \\ \hline
11         & 0.061     & 0.049 & 0.000 & 0.000   \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{Path Cost Ratio at worst case in Complete Graph}
\label{tab:Complete_worst}
\begin{tabular}{|l|l|l|l|l|}
\hline
Order      & Insertion & Swap  & GA    & Swap+GA \\ \hline
5          & 1.195     & 1.000 & 1.000 & 1.000   \\ \hline
6          & 1.262     & 1.198 & 1.000 & 1.000   \\ \hline
7          & 1.260     & 1.250 & 1.000 & 1.000   \\ \hline
8          & 1.407     & 1.407 & 1.000 & 1.000   \\ \hline
9          & 1.392     & 1.328 & 1.000 & 1.000   \\ \hline
10         & 1.379     & 1.370 & 1.000 & 1.000   \\ \hline
11         & 1.482     & 1.337 & 1.012 & 1.001   \\ \hline
\end{tabular}
\end{table}

==> tsp_incomplete_graph.tex <==
\begin{table}[]
\caption{Average Path Cost in Incomplete Graph}
\label{tab:Incomplete_avg_cost}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Order      & Insertion & Swap  & GA    & Swap+GA & BruteForce \\ \hline
5          & 1.069     & 1.016 & 1.003 & 1.004   & 1.000      \\ \hline
6          & 1.092     & 1.034 & 1.005 & 1.005   & 1.000      \\ \hline
7          & 1.110     & 1.041 & 1.005 & 1.005   & 1.000      \\ \hline
8          & 1.133     & 1.056 & 1.005 & 1.006   & 1.000      \\ \hline
9          & 1.149     & 1.068 & 1.005 & 1.007   & 1.000      \\ \hline
10         & 1.166     & 1.079 & 1.004 & 1.006   & 1.000      \\ \hline
11         & 1.186     & 1.093 & 1.006 & 1.008   & 1.000      \\ \hline
12         & 1.248     & 1.143 & 1.023 & 1.021   & 1.000      \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Optimal Path ratio in Incomplete Graph}
\label{tab:Incomplete_optimal}
\begin{tabular}{|l|l|l|l|l|}
\hline
Order      & Insertion & Swap    & GA      & Swap+GA \\ \hline
5          & 89.867    & 100.000 & 100.000 & 100.000 \\ \hline
6          & 77.300    & 94.333  & 100.000 & 100.000 \\ \hline
7          & 64.433    & 84.167  & 100.000 & 100.000 \\ \hline
8          & 53.733    & 75.900  & 100.000 & 100.000 \\ \hline
9          & 41.800    & 66.300  & 100.000 & 100.000 \\ \hline
10         & 33.100    & 54.600  & 100.000 & 100.000 \\ \hline
11         & 26.071    & 48.233  & 99.958  & 99.958  \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{Standard Deviation of path cost ratio in Incomplete graph}
\label{tab:Incomplete_std_diff}
\begin{tabular}{|l|l|l|l|l|}
\hline
Order      & Insertion & Swap  & GA    & Swap+GA \\ \hline
5          & 0.018     & 0.000 & 0.000 & 0.000   \\ \hline
6          & 0.030     & 0.013 & 0.000 & 0.000   \\ \hline
7          & 0.038     & 0.023 & 0.000 & 0.000   \\ \hline
8          & 0.046     & 0.032 & 0.000 & 0.000   \\ \hline
9          & 0.053     & 0.037 & 0.000 & 0.000   \\ \hline
10         & 0.060     & 0.047 & 0.000 & 0.000   \\ \hline
11         & 0.061     & 0.049 & 0.000 & 0.000   \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{Path Cost Ratio at worst case in Incomplete Graph}
\label{tab:Incomplete_worst}
\begin{tabular}{|l|l|l|l|l|}
\hline
Order      & Insertion & Swap  & GA    & Swap+GA \\ \hline
5          & 1.195     & 1.000 & 1.000 & 1.000   \\ \hline
6          & 1.262     & 1.198 & 1.000 & 1.000   \\ \hline
7          & 1.260     & 1.250 & 1.000 & 1.000   \\ \hline
8          & 1.407     & 1.407 & 1.000 & 1.000   \\ \hline
9          & 1.392     & 1.328 & 1.000 & 1.000   \\ \hline
10         & 1.379     & 1.370 & 1.000 & 1.000   \\ \hline
11         & 1.482     & 1.337 & 1.012 & 1.001   \\ \hline
\end{tabular}
\end{table}
